Asymptotic Rate Analysis for Impairments-Aware Multi-Carrier FD Massive MIMO Relay Networks utilizing MRT/MRC Strategy

In this paper, we analyze the asymptotic rate for a multi-carrier (MC) full-duplex (FD) massive multiple input multiple output (mMIMO) decode and forward (DF) relay system which serves multiple MC single-antenna half-duplex (HD) nodes. We take into account the impact of hardware distortions resulting in residual self-interference (SI) and inter-carrier leakage (ICL) as well as the impact of imperfect channel state information (CSI). We derive the asymptotic rate expression of our system employed with maximum ratio transmitting (MRT)/ maximum ratio combining (MRC) strategy when the number of the antenna becomes large (goes to $\infty$). It is noticed that the impact of hardware distortion becomes remarkable in a large-scale antenna array regime. On contrary to the effect of multi-user interference and receiver noise, which vanishes as the number of relay antenna goes to infinity, the residual SI and ICL caused by the hardware impairments remains in the MC system.

==> acronyms.tex <==
\chapter*{List of Acronyms}
\addcontentsline{toc}{chapter}{List of Acronyms}

% number of X defines indentation
\begin{acronym}[XXXXXXXX]
    \acro{3GPP}{3rd Generation Partnership Project}  
    \acro{4G}{fourth-generation} 
    \acro{5G}{fifth-generation} 
    \acro{ADC}{analog to digital converter}
    \acro{AF}{amplify and forward}
    \acro{AGC}{automatic gain control}
    \acro{AQCP}{alternating quadratic convex program}
    \acro{BS}{base station}
    \acro{CDMA}{Code Division Multiple Access}
    \acro{CP}{cyclic prefix}
	\acro{CSI}{channel state information}
    \acro{CT}{computational time} 
    \acro{CQP}{conic quadratic program}
    \acro{DAC}{digital to analog converter}
    \acro{DC}{difference-of-convex}
    \acro{DF}{decode and forward}
    \acro{DL}{direct link}
    \acro{DuC}{Dual Connectivity}
    \acro{EE}{Energy Efficiency}
    \acro{FBMC}{Filter Bank Multi Carrier}
    \acro{FD}{full-duplex}
    \acro{FDMA}{Frequency Division Multiple Access}
    \acro{GFDM}{Generalised Frequency Division Multiplexing}
    \acro{HD}{half-duplex}
    \acro{ICL}{inter-carrier leakage}
    \acro{i.i.d.}{independent and identically distributed}
    \acro{JC}{Joint Carrier}
    \acro{KKT}{Karush–Kuhn–Tucker}
    \acro{LD}{less distortion}
    \acro{LMMSE}{linear minimum mean square error}
    \acro{LOS}{line of sight}
    \acro{LTE}{long time evolution}
    \acro{mMIMO}{massive multiple input multiple output}
    \acro{MC}{multi-carrier}
    \acro{MIMO}{multiple input multiple output}
    \acro{mixed-OFDM}{mixed-orthogonal frequency division multiplexing}
    \acro{MeNB}{Master evolved Node B}
    \acro{MMSE}{minimum mean square error}
    \acro{MRC}{maximum ratio combining} 
    \acro{MRT}{maximum ratio transmitting}
    \acro{ND}{non-distortion}
    \acro{NLOS}{non-line of Sight}
    \acro{NOMA}{non-orthogonal multiple access}
    \acro{NR}{New Radio}
    \acro{OFDM}{orthogonal frequency division multiplexing}
    \acro{ODL}{only direct link}
    \acro{ORL}{only relay link}
    \acro{OVSF}{orthogonal variable spreading factor}
    \acro{PC}{Per Carrier} 
    \acro{QoS}{quality of service}
    \acro{RF}{radio frequency}
    \acro{RL}{relay link} 
    \acro{RS}{rate-splitting}
    \acro{RSM}{right-singular matrix}
    \acro{SA}{single antenna}
    \acro{SeNB}{Secondary evolved Node B}
    \acro{SI}{self-interference}
    \acro{SIA}{successive inner approximation} 
    \acro{SIC}{self-interference cancellation}
    \acro{SIMO}{single input multiple output}
    \acro{SINR}{signal to interference plus noise ratio}
    \acro{SNR}{signal to noise ratio}
    \acro{SuIC}{successive interference cancellation}
    \acro{SWIPT}{simultaneous wireless information and power transfer} 
    \acro{TDMA}{Time Division Multiple Access}
    \acro{TDD}{time division duplex}
    \acro{UE}{user equipment}
    \acro{Wo-CSI}{without channel state information error}
    \acro{ZF}{zero-forcing}
    \acro{ZFT}{zero-forcing transmitting}
    \acro{ZFR}{zero-forcing  receiving}
\end{acronym}

